Switch Point biased Self-Training: Re-purposing Pretrained Models for Code-Switching

Code-switching (CS), a ubiquitous phenomenon due to the ease of communication it offers in multilingual communities still remains an understudied problem in language processing. The primary reasons behind this are: (1) minimal efforts in leveraging large pretrained multilingual models, and (2) the lack of annotated data. The distinguishing case of low performance of multilingual models in CS is the intra-sentence mixing of languages leading to switch points. We first benchmark two sequence labeling tasks -- POS and NER on 4 different language pairs with a suite of pretrained models to identify the problems and select the best performing model, char-BERT, among them (addressing (1)). We then propose a self training method to repurpose the existing pretrained models using a switch-point bias by leveraging unannotated data (addressing (2)). We finally demonstrate that our approach performs well on both tasks by reducing the gap between the switch point performance while retaining the overall performance on two distinct language pairs in both the tasks. Our code is available here: https://github.com/PC09/EMNLP2021-Switch-Point-biased-Self-Training.

==> sections/experiments.tex <==




% We  apply  Roman-to-Devanagari  transliteration  on  the  Hindi-Englishdatasets since the multilingual models are trained with data using that form. Table 1 shows the num-ber of tokens of each language for each dataset.We classify the language with more tokens as theML  and  the  other  as  the  EL.  We  replace  userhashtags and mentions with<USR>, emoji with<EMOJI>, and URL with<URL>for models thatuse  word-embeddings,  similar  to  Winata  et  al.(2019a).  We evaluate our model with the microF1 score for NER and accuracy for POS tagging,following Aguilar et al. (2020a).

%\subsection{Models}

\iffalse
We performed sequence tagging on different transformer based models as described below.

\begin{itemize}
    \item \textbf{BERT} \cite {devlin2018bert} :  The original BERT model was trained using Masked Language Modelling (MLM) and Next Sentence Prediction (NSP) objectives and has approximately 110M parameters. We use the uncased-base implementation for our work.
    
    \item \textbf{mBERT} \cite{devlin2018bert}:  This is a multilingual BERT model trained on 104 languages and has approximately 179M parameters. We again use the uncased-base model for our work.
    
    \item \textbf{Distill mBERT} \cite{sanh2019distilbert}: This multilingual model is initialised with weights from multilingual BERT model but with the help of knowledge distillation in pretraining phase, the model size reduced significantly. 
    
    
    \item \textbf{XLM-RoBERTa}\cite{conneau2019unsupervised}:This is  a multilingual  RoBERTa modeltrained on 100 languages and has approx-imately 270M parameters. The XLM-RoBERTamodel is trained large multilingual corpusof 2.5TB of web crawled data.  We use theuncased-base XLM-RoBERTa model.
    
    
    \item\textbf{Char-BERT}\cite{boukkouri2020characterbert} : This model produces word level contextual representation by attending to the characters of each input token.Thus, instead of relying on wordpieces, it uses a CharacterCNN module similar to ELMO to capture unknown and misspelled words.
    

\end{itemize}
\fi 
    

%\subsection{Setup}

%In the majority of our approaches, we perform task adaptive ﬁne-tuning on BERT, mBERT , XLM-Roberta and character BERT for few  epochs on an Nvidia GeForce GTX 1070 GPU. We experiment with batch sizes of 8,16, and 32, and learning rates between 1e-5 and 5e-5. We primarily used Pytorch and Huggingface library for implementing different models.
%For some models, we observed variation in performance on test set based on subset of data used for training. To overcome this, we did 5 fold cross validation where there were no pre-defined train, dev and test data splits. 


==> sections/results.tex <==

\subsection{Iterative Data Augmentation}



==> tables/lang-aware-multi-task.tex <==
\begin{table*}
\small
\centering
\begin{tabular}{llllll}
\hline
\textbf{Model} & \textbf{POS-En-HI-Twitter} & \textbf{POS-EN-HI-UD} & \textbf{NER-EN-HI-Twitter} & \textbf{NER-EN-ES-Twitter}  \\
\hline
M-BERT (Our baseline) & 89.27 & 87.67 & 74.2 & 60.12 \\
M-BERT (Language at Input) & 89.74 & 87.96 & 75.38 & 61.46 \\
M-BERT (Language at Output) & 88.89 & 86.47 & 74.01 & 60.20 \\
char-BERT (Our baseline) & 90.89 & 90.23 &  77.24 & 65.72 \\
char-BERT (Language at Input) & 91.02 & 90.93 & 77.43 & 66.34\\
char-BERT (Language at Output) & 90.25 & 89.29 & 77.12 & 66.01 \\


\hline
\end{tabular}
\caption{\label{citation-guide}
Performance comparison for single vs  multi-task training- POS(Accuracy) and NER (F1)
}
\end{table*}

==> tables/ner.tex <==






\begin{table}
\tiny
\centering
\begin{tabular}{llllll}
\hline
\textbf{Model} & \textbf{EN-HI-Twitter} & \textbf{EN-ES-Twitter} & \textbf{MSA-EA} \\
\hline
Baseline & 78.21  & 69.17  & 71.61 \\
eng-BERT & 65.93 & 55.12 & 74.13 \\
M-BERT & 74.2 & 60.12 & 79.73 \\
Distill M-BERT & 67.26 & 62.67 & 77.28 \\
XLM-ROBERTa & 73.34 & 66.12 & 77.68 \\
char-BERT & 77.24 & 65.72 & 74.46  \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Performance of different multilingual models for various NER tagging datasets (F1)
}
\end{table}



